Do All Good Actors Look The Same? Exploring News Veracity Detection Across The U.S. and The U.K

A major concern with text-based news veracity detection methods is that they may not generalize across countries and cultures. In this short paper, we explicitly test news veracity models across news data from the United States and the United Kingdom, demonstrating there is reason for concern of generalizabilty. Through a series of testing scenarios, we show that text-based classifiers perform poorly when trained on one country's news data and tested on another. Furthermore, these same models have trouble classifying unseen, unreliable news sources. In conclusion, we discuss implications of these results and avenues for future work.

==> tex/labels_legend_table.tex <==
\newgeometry{left=2cm, top=1.4cm}

\begin{table*}[!ht]
    \fontsize{9}{9.2}\selectfont  % fontsize, spacing
    \renewcommand{\arraystretch}{1.4}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[t]{L{3.6cm}lL{10.4cm}C{2.5cm}}
        \textbf{Section} & & \textbf{Description} \hfill (NewsGuard points) & \textbf{Coloring} \\ \hline
        %
        NewsGuard 
        & ~~1. & Does not repeatedly publish false content \hfill (22.0)  & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~2. & Gathers and presents information responsibly \hfill (18.0) &  \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~3. & Regularly corrects or clarifies errors \hfill (12.5)  &                                 \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~4. & Handles the difference between news and opinion responsibly \hfill (12.5)  &            \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~5. & Avoids deceptive headlines \hfill (10.0) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~6. & Website discloses ownership and financing \hfill (7.5) &                               \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~7. & Clearly labels advertising \hfill (7.5) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~8. & Reveals who's in charge, including any possible conflicts of interest \hfill (5.0) &   \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~9. & Provides information about content creators \hfill (5.0) &                             \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& 10. & Aggregated \texttt{score} computed from 1-9 & \includegraphics[width=1.6ex]{fig/colors/green.pdf} - \includegraphics[width=1.6ex]{fig/colors/purple.pdf} ~~ \\
    	& 11. & Column 10 thresholded at 60 points &
    	\includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
    	% 
    	Pew Research Center 
    	& 12. & Trust from consistently-liberals & \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 13. & Trust from mostly-liberals & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 14. & Trust from mixed groups & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 15. & Trust from mostly-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 16. & Trust from consistently-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 17. & Aggregated trust from 12-16 & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Wikipedia 
        & 18. & Existence of source on Wikipedia's list of fake news sources & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Open Sources 
        & 19. & Marked reliable & \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\
        & 20. & Marked blog & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 21. & Marked clickbait & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 22. & Marked rumor & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 23. & Marked fake & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 24. & Marked unreliable & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 25. & Marked biased & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 26. & Marked conspiracy & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 27. & Marked hate speech & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 28. & Marked junk science & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 29. & Marked political & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 30. & Marked satire & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 31. & Marked state news & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\ \hline
        %
        Media Bias / Fact Check 
        & 32. & Factual reporting from 5 (good) down to 1 (bad) & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 33. & Special label; conspiracy, pseudoscience or questionable source (purple), and satire (orange) &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 34. & Political leaning / bias from left to right. & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        Allsides 
        & 35. & Political leaning / bias & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        BuzzFeed
        & 36. & Political leaning / bias, but only left and right &
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        PolitiFact
        & 37. & Has brought story labelled as "pants on Fire!" &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 38. & Has brought story labelled as false &
        \includegraphics[width=1.6ex]{fig/colors/purple2_grey.pdf} \\
        & 39. & Has brought story labelled as mostly false &
        \includegraphics[width=1.6ex]{fig/colors/purple_grey2.pdf} \\
        & 40. & Has brought story labelled as half-true &
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 41. & Has brought story labelled as mostly true &
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} \\
        & 42. & Has brought story labelled as true &
        \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\ \hline
        %
        Alexa Ranking & & The Alexa ranking of the source. & Numerical \\ \hline
        %
        \# Articles & & The number of articles collected from the source. & Numerical \\ \hline
        %
        First Observed & & The date of first articles collected from the source. & dd-mm-yyyy \\ \hline
    \end{tabular}
    \caption{Details of the information for sources found in tables \ref{tab:source_labels1}, \ref{tab:source_labels2} and \ref{tab:source_no_labels}. We generally use green-to-purple for good-to-poor reliability/credibility, with grey as inconclusive. For bias we use blue-to-red for left-to-right bias, with grey as unbiased. Orange is used for special cases. In NewsGuard data it represents missing information, in Open Sources it marks auxiliary labels and for Media Bias / Fact Check it marks satire. }
    \label{tab:labelling_explanations}
\end{table*}

\restoregeometry

